On the Second-Order Asymptotics of the Hoeffding Test and Other Divergence Tests

Consider a binary statistical hypothesis testing problem, where $n$ independent and identically distributed random variables $Z^n$ are either distributed according to the null hypothesis $P$ or the alternative hypothesis $Q$, and only $P$ is known. A well-known test that is suitable for this case is the so-called Hoeffding test, which accepts $P$ if the Kullback-Leibler (KL) divergence between the empirical distribution of $Z^n$ and $P$ is below some threshold. This work characterizes the first and second-order terms of the type-II error probability for a fixed type-I error probability for the Hoeffding test as well as for divergence tests, where the KL divergence is replaced by a general divergence. It is demonstrated that, irrespective of the divergence, divergence tests achieve the first-order term of the Neyman-Pearson test, which is the optimal test when both $P$ and $Q$ are known. In contrast, the second-order term of divergence tests is strictly worse than that of the Neyman-Pearson test. It is further demonstrated that divergence tests with an invariant divergence achieve the same second-order term as the Hoeffding test, but divergence tests with a non-invariant divergence may outperform the Hoeffding test for some alternative hypotheses $Q$. Potentially, this behavior could be exploited by a composite hypothesis test with partial knowledge of the alternative hypothesis $Q$ by tailoring the divergence of the divergence test to the set of possible alternative hypotheses.

==> apdx_compchino.tex <==
\section{Proof of Lemma  \ref{lem:chi-normal}} \label{proofcompchino}
Consider any eigenvalue $\lambda_{j}$  of the positive-definite matrix $\bm{B}= \bm{\Sigma}_{\mathbf{P}}^{-1/2}\bm{A}_{D,\mathbf{P}} \bm{\Sigma}_{\mathbf{P}}^{-1/2}$. Let $Y_{1},\cdots,Y_{k-1}$ be i.i.d. standard Normal random variables. Then, for \mbox{$y \geq 0$},
\begin{equation}
	\mathsf{Q}_{\mathcal{N}}\left( \frac{y}{\sqrt{\lambda_{j}}}\right) 	<  \text{Pr} \left( Y_{j}^{2} \geq  \frac{y^{2}}{\lambda_{j}}\right)  \leq \text{Pr} \left( \sum_{i=1}^{k-1}  \lambda_{i}Y_{i}^{2} \geq  y^{2}\right) = \mathsf{Q}_{\chi^{2}_{\bm{\lambda},k-1}}(y^{2}) \label{eq:qcomp1}
\end{equation}
where the first inequality follows because \[\text{Pr}( Y_{j}^{2} \geq  d^{2})=\text{Pr}(|Y_j| \geq d) = 2 \mathsf{Q}_{\mathcal{N}}(d),\; d \geq 0\] and the second inequality follows because $\lambda_{j}Y_j^2 \leq \sum_{i=1}^{k-1} \lambda_{i} Y_i^2$ with probability one. Let $y$ be such that \mbox{$ \mathsf{Q}_{\chi^{2}_{\bm{\lambda},k-1}}(y^{2})=\epsilon$}. Since $y \mapsto\mathsf{Q}_{\mathcal{N}}(y)$ is strictly decreasing, we obtain from \eqref{eq:qcomp1} that there exists a \mbox{$y' < \frac{y}{\sqrt{\lambda_{j}}}$} such that \mbox{$\mathsf{Q}_{\mathcal{N}}(y')=\epsilon$}. It then follows that $\mathsf{Q}_{\mathcal{N}}^{-1}(\epsilon)  =y'$ which implies that
\begin{equation}
	\mathsf{Q}_{\mathcal{N}}^{-1}(\epsilon)  < \frac{1}{\sqrt{\lambda_{j}}}\sqrt{\mathsf{Q}^{-1}_{\chi^{2}_{\bm{\lambda},k-1}}(\epsilon)}, \quad \text{for any}\quad  j \in \left\lbrace 1,\cdots,k-1\right\rbrace . \label{eq:qcomp2}
\end{equation}
Next, we note that
\begin{equation}
	\frac{\mathbf{c}^{\mathsf{T}} \bm{A}_{D,\mathbf{P}} ^{-1} \mathbf{c}}{V(P \| Q)} =\frac{\mathbf{c}^{\mathsf{T}} \bm{A}_{D,\mathbf{P}} ^{-1} \mathbf{c}}{	\mathbf{c}^{\mathsf{T}} \bm{\Sigma}^{-1}_{\mathbf{P}} \mathbf{c}}
\end{equation}
Using the transformation $\tilde{\mathbf{c}}=\bm{\Sigma}_{\mathbf{P}}^{-1/2} \mathbf{c}$, we obtain that
\begin{eqnarray}
	\frac{\mathbf{c}^{\mathsf{T}} \bm{A}_{D,\mathbf{P}} ^{-1} \mathbf{c}}{V(P \| Q)} &= &\frac{\tilde{\mathbf{c}}^{\mathsf{T}}   \bm{\Sigma}_{\mathbf{P}}^{1/2}\bm{A}_{D,\mathbf{P}} ^{-1}   \bm{\Sigma}_{\mathbf{P}}^{1/2}\tilde{\mathbf{c}}}{	\tilde{\mathbf{c}}^{\mathsf{T}} \tilde{\mathbf{c}}} \notag\\
	&=& \frac{\tilde{\mathbf{c}}^{\mathsf{T}}  \bm{B}^{-1}\tilde{\mathbf{c}}}{\tilde{\mathbf{c}}^{\mathsf{T}} \tilde{\mathbf{c}}}.\label{eq:quadbound1} 
\end{eqnarray}
It then follows from the Rayleigh-Ritz theorem \cite[Theorem 4.2.2]{RJ90} that
\begin{eqnarray}
	\frac{1}{\lambda_{\textnormal{max}}} \leq 	 \frac{\tilde{\mathbf{c}}^{\mathsf{T}}  \bm{B}^{-1}\tilde{\mathbf{c}}}{\tilde{\mathbf{c}}^{\mathsf{T}} \tilde{\mathbf{c}}}\leq \frac{1}{\lambda_{\textnormal{min}}}. \label{eq:quadbound3} 
\end{eqnarray}
where  $\lambda_{\textnormal{min}} $ and $\lambda_{\textnormal{max}} $ are the minimum and the maximum of the set of all eigenvalues of the positive-definite matrix $\bm{B}$. Together with \eqref{eq:quadbound1}, this yields
\begin{eqnarray}
	\frac{1}{\sqrt{\lambda_{\textnormal{max}}}} \leq 		\frac{ \sqrt{\mathbf{c}^{\mathsf{T}} \bm{A}_{D,\mathbf{P}}^{-1} \mathbf{c}}}{\sqrt{V(P \| Q)}} \leq \frac{1}{\sqrt{\lambda_{\textnormal{min}}}}. \label{eq:quadbound4} 
\end{eqnarray}
Combining  \eqref{eq:qcomp2} and \eqref{eq:quadbound4}, we obtain the desired inequality: 
\begin{eqnarray}
	\sqrt{\mathbf{c}^{T} \bm{A}_{D,\mathbf{P} }^{-1} \mathbf{c}} \sqrt{\mathsf{Q}^{-1}_{\chi^{2}_{\bm{\lambda},k-1}}(\epsilon)}&\geq&  \frac{\sqrt{V(P \| Q)} \sqrt{\mathsf{Q}^{-1}_{\chi^{2}_{\bm{\lambda},k-1}}(\epsilon)}}{\sqrt{\lambda_{\textnormal{max}}}} \notag \\
	& >& 	\mathsf{Q}_{\mathcal{N}}^{-1}(\epsilon) \sqrt{V(P \| Q)}. \label{eq:quadbound5} 
\end{eqnarray} 

==> notations.tex <==
\section{Notations}




%{\color{red}  
%In this manuscript, we use the following conventions in notations:
% \begin{itemize}
%	\item  General probability $k$-vector : $T=(T_{1},\cdots,T_{k})^{\mathsf{T}}$, other symbols used are $R, \Gamma, T', Q', T_{n}, T_{n}^{*}$. 
%	\item Chosen coordinate $k-1$-vector of any $T \in \mathcal{P}(\mathcal{Z}) $, we use boldface letters  $\mathbf{T}, \mathbf{R}, \mathbf{\Gamma}, \mathbf{T}', \mathbf{Q}', \mathbf{T}_{n}, \mathbf{T}_{n}^{*}$.
%	\item Any $\Bbb R^{d}$-valued random vector: $\mathbf{X}^{d}$, symbols used are $\mathbf{X}_{n}^{k-1}, \mathbf{Y}^{k-1}, \mathbf{V}^{k-1}, \mathbf{Z}^{k-1}, \mathbf{V}_{n}^{k-1}$.
%	\item Any real vector in $\Bbb R^{d}$: $\mathbf{x}=(x_{1},\cdots,x_{d})^{\mathsf{T}}$ or $\bm{\delta}=(\delta_{1},\cdots,\delta_{k-1})^{\mathsf{T}}$, 
%	other symbols used are $\mathbf{v}, \mathbf{c}, \tilde{\mathbf{c}}, \mathbf{a},\bar{\mathbf{x}}, \bar{\mathbf{y}}$, $ \bm{\varepsilon}, \bar{\bm{\delta}},\bm{\theta}$. 
%\end{itemize}}
%

